Glowing in the Dark Uncovering IPv6 Address Discovery and Scanning Strategies in the Wild

In this work we identify scanning strategies of IPv6 scanners on the Internet. We offer a unique perspective on the behavior of IPv6 scanners by conducting controlled experiments leveraging a large and unused /56 IPv6 subnet. We selectively make parts of the subnet visible to scanners by hosting applications that make direct or indirect contact with IPv6- capable servers on the Internet. By careful experiment design, we mitigate the effects of hidden variables on scans sent to our /56 subnet and establish causal relationships between IPv6 host activity types and the scanner attention they evoke. We show that IPv6 host activities e.g., Web browsing, membership in the NTP pool and Tor network, cause scanners to send a magnitude higher number of unsolicited IP scans and reverse DNS queries to our subnet than before. DNS scanners focus their scans in narrow regions of the address space where our applications are hosted whereas IP scanners broadly scan the entire subnet. Even after the host activity from our subnet subsides, we observe persistent residual scanning to portions of the address space that previously hosted applications

==> Makefile <==
# Makefile for LaTeX files
# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile
# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.
# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo
# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 
# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 
# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $
LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"
DATE=$(shell date +%Y-%m-%d)
COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false
# These are OK
SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)
# These are not
#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))
define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef
define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef
define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef
define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef
define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef
define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef
all 	: $(TRG)
.PHONY	: all show clean ps pdf showps veryclean
clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)
veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~
# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 
include $(SRC:.tex=.d)
# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)
$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@
#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)
show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done
showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done
ps	: $(PSF) 
pdf	: $(PDF) 
# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)
######################################################################
# Define rules for EPS source files.
# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12
#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))

==> tex/methodology.tex <==
% \section{Methodology}\label{sec:methodology}
% In this section, we explain the experimental setup and data collection methods we used in our study. For the entirety of our experiments, we used a previously unused (and unrouted?) /56 IPv6 prefix present inside a university wide allocation. The following subsections detail the division and usage of this address space to answer our proposed research questions. 
% //

% Talk about how we cleaned up our traffic? Making sure we dont count IP addresses we contacted ourselves?


% \subsection{Measuring the prevalence of scanning activity in IPv6}
% Longitudinal study spanning 6 months. collected all pcap traffic and dns logs for the entirety of our study. started collection as soon as the space was routed. didnt run anything for the first few weeks to establish a base rate. what are the highlevel characteristics of the incoming traffic we see? Geographical regions? Type of traffic - TCP, ICMP, UDP? CDFs of general trends? how many of these IPs do we see in the abuse dataset? Maybe do a longitudnal graph for that if data is available? 


% \subsection{Characterizing the technqiues used by scanners to find active hosts}
% ran services only in one of the four /58s. leaked low bit addresses and random addresses. analyzed incoming scanning behavior; sequential or heuristic based? do scanners use a single ip address to scan or change their addresses or use multiple IPs from assigned subnets. are the scans restricted to subnets which were leaked or did the neighbors also receive scanning activity? was there a difference? what was the perceived subnet size by these scanners (using dns data). do scanners use previously studied technqiues? can we establish if two or more scanners used a similar technique to scan our networks.


% \subsection{Understanding how host activity affects scanning behavior and prevalence}

% \subsubsection{Alexa top 10k websites crawler}
% \subsubsection{Crawling open IPv6 DNS resolvers}
% \subsubsection{NTP pool servers}
% \subsubsection{NTP public servers}
% \subsubsection{Tor relay}
% \subsubsection{DNS zone files}


\subsection{Methodology}
\label{sec:methodology}
% What are we doing?
% Cause: Measuring the effect of \emph{IPv6 host activity} on the type and 
% volume of scanning activity it attracts on the Internet.
% Effect: we end up leaking our address to different types of v6 scanners.

% Considerations we had before starting the measurements
% 1. We need a representative block of v6 address space so we can claim our
% results generalize.

% 2. It should be an unused address space so we could identify the scanning
% activity resulting from our experiments. Here we got a block of IPv6
% addresses that were previously un-announced (but owned by UIowa) to the Internet.
% This means that no legitimate traffic could be received in this address space
% This is an Internet darkspace~\cite{caidatelescope}. Uiowa was not using 
% this address space. Where in UIowa's allocation was this /56.

% 3. Once the address block got allocated to us (EXACT STEPS that IT performed
% to allocate this to us. was it BGP announcement, what else?), we observed
% unsolicited traffic that we got. <Summarize in 2 lines, what kind of traffic
% we saw in the 2 months when there was no host activity>.
% Observed three main scanners from X Y Z autonomous systems with mild 
% recurring activity. <Protocol, port, how often did each of the 3 scanners
% come to us for>

We conduct a longitudinal study to measure the effects of host activity on 
scanning in IPv6 networks. To achieve this, we simulate different 
kinds of host activity in a previously unrouted and unallocated /56 IPv6 prefix.
\\
\textbf{Where was our /56 IPv6 prefix located?} Our /56 IPv6 prefix was part of a larger /48 allocation for a university network. 
\\
\textbf{How did we divide our /56 IPv6 prefix?} Addresses inside a /56 IPv6 prefix can theoretically be assigned to $2^{72}$ distinct hosts. However, according to standard practice, an IPv6 address comprises of two parts; a 64 bit subnet identifier and a 64 bit interface identifier \cite{RFC4291}. 
A typical IPv6 host address resides in 64 bits of host address space \cite{RFC4862}. Following this best practice,
our allotted /56 IPv6 space be divided into a possible $2^{64 - 56} = 2^8$ distinct host address spaces. For purposes of 
analyzing scanning patterns and behaviors in neighboring host address spaces, we divide the /56 address space into 4 regions 
of /58 address spaces. For the entirety of our experiment, we only use host addresses from one of the four /58 IPv6 prefixes.
\\
\textbf{When was this prefix first used?}
This prefix assigned to us was not the originator of any network traffic before the start of our experiments. The prefix was assigned to us in \textit{November 2020} but the first experiment started in \textit{March 2021.} This allowed us to analyze how regions of little to no activity get scanned and how this behavior changes once host activity is simulated. 

\textbf{How did we simulate host activity?}
Following the initial $3$ month period of inactivity, we conducted the following experiments to simulate host activity:
\begin{itemize}
	\item Alexa top 10k websites crawler 
	\item DNS open resolver crawler
	\item NTP pool server
	\item NTP public sever
	\item Tor middle relays
	\item DNS zone files 
\end{itemize}
\textbf{Figure 1} shows when each of these experiments were run during the duration of our experiments. Each experiment was run exclusively. However, 4 simultaneous instances were run for each experiment with each instance allotted a different IPv6 address. For each experiment, 2 instances were run using a lower-byte interface ID (IID) address and the other 2 instances were run using a random IID address. A lower-byte IID address has all 0s in the interface ID part of the IPv6 address except for the last byte e.g \textit{2001:d00f:1:2::23} which is an abbreviated version of \textit{2001:d00f:1:2:0000:0000:0000:0023}. On the other hand, a random IID address does not have a defined pattern in the interface ID part of the address e.g \textit{2001:d00f:1:2:83c4:4c0:bb21:8766} All 4 addresses for a single experiment were placed in distinct /64 subnets that were chosen randomly. All 4 /64 subnets for a single experiment had a gap of at least 1 /64 prefix between them. This setup is depicted in \textbf{Figure 2}. 

\textbf{Alexa top 10k crawlers.}  We used OpenWPM to conduct of the Alexa top 10k websites. The AAAA DNS records were collected for all the top 10k websites prior to crawls. We ran four instances of OpenWPM crawlers that ran simultaneously visiting each website with a valid AAAA record. On average, ~2600 websites returned valid AAAA records before the start of each crawl. Using OpenWPM allowed us to conduct full web page crawls  

\textbf{DNS open resolvers crawlers.} This experiment involved querying open DNS resolvers for an IPv6 domain. We collected a list of ~9k open DNS resolvers. These resolvers were queried simultaneously for the AAAA DNS record of \textit{www.google.com} using the 4 addresses allotted to this experiment. Each resolver was queried once every day (at most 3 times for a successful response) for the entirety of the experiment.

\textbf{NTP pool servers.} This experiment consisted of setting up 4 instances of NTP pool servers. \textit{should i put in stats about the pool servers  and the config?}

\textbf{NTP public servers.}

\textbf{Tor relays.} Talk about bandwidth? middle relay? People who used our relays? 

\textbf{DNS zone files.} To conduct this experiment, we set up 4 domains; 2 each with a \textit{.com} and \textit{.net} TLD. The AAAA records of all 4 domains were pointed to 4 distinct IPv6 addresses in our /56 IPv6 prefix. \textit{Should i explain here how dns zone files work?}
\\
\textbf{What data did we collect?}
Throughout the length of our experiment, we capture:
\begin{itemize}
	\item All network traffic destined for our /56 IPv6 prefix
	\item Logs of DNS PTR record queries made for IPs that reside inside our /56 IPv6 prefix
\end{itemize}   

\textbf{How did we collect this data?}
We ran tcpdump to capture all traffic originating from and destined to our /56 IPv6 prefix. To collect DNS PTR record queries, we ran an authoritative DNS server which served all domains assigned to our IP addresses with a TTL of 1. This made sure that most PTR record queries were not cached and indeed reached our DNS server.



==> tex/our_dataset.tex <==
% \section{Experimentation setup and the IPv6 scanning dataset}\label{sec:our_dataset}


% In this section, we detail the experimentation setup and data collection methods we used to curate the dataset for this study. 

% \subsection{Experimentation setup}
% In this study, we conducted a longitudinal study spanning over 6 months to measure the effects of host activity on scanning in IPv6 networks. To achieve this, we simulate different kinds of host activity in a previously unrouted and unallocated /56 IPv6 prefix. This /56 prefix is part of a /48 IPv6 address space allotted to a university. 
% \\
% \\
% \textbf{Division of the /56 IPv6 address block}
% \\
% Addresses inside a /56 IPv6 prefix can theoretically be assigned to $2^{72}$ distinct hosts. However, according to standard practice, an IPv6 address comprises of two parts; a 64 bit subnet identifier and a 64 bit interface identifier \cite{RFC4291}. 
% A typical IPv6 host address resides in 64 bits of host address space \cite{RFC4862}. Following this best practice,
% our allotted /56 IPv6 space be divided into a possible $2^{64 - 56} = 2^8$ distinct host address spaces. For purposes of 
% analyzing scanning patterns and behaviors in neighboring host address spaces, we divide the /56 address space into 4 regions 
% of /58 address spaces. For the entirety of our experiment, we only use host addresses from one of the four /58 IPv6 prefixes.
% \textbf{Figure 2} shows the division of the /56 IPv6 address block.
% \\
% \\
\textbf{Simulating host activity}
\\
This /56 IPv6 prefix was previously unused and hence no traffic was previously originated from this address space. This allowed us to analyze IPv6 scanning behavior in regions of little to no activity and how this behavior changes over time with different host activity. We were allotted our /56 IPv6 prefix in \textit{November 2020}. For the first $3$ months, we did not simulate any host activity to observe how unused regions of IPv6 address space receive scanning activity. Following this initial $3$ month period, we conducted the following experiments to simulate host activity:
\begin{itemize}
	\item Alexa top 10k websites crawler 
	\item DNS open resolver crawler
	\item NTP pool server
	\item NTP public sever
	\item Tor middle relays
	\item DNS zone files 
\end{itemize}
\textbf{Figure 1} shows when each of these experiments were run during the duration of our experiments. Each experiment was run exclusively. However, 4 simultaneous instances were run for each experiment with each instance allotted a different IPv6 address. For each experiment, 2 instances were run using a lower-byte address and the other 2 instances were run using a random IID address. All 4 addresses for a single experiment were placed in distinct /64 subnets that were chosen randomly. All 4 /64 subnets for a single experiment had a gap of at least 1 /64 prefix between them. This setup is depicted in \textbf{Figure 2}. 
\\ 
\textbf{Alexa top 10k crawlers.}  We used OpenWPM to conduct full web page crawls of the Alexa top 10k websites. The AAAA DNS records were collected for all the top 10k websites prior to crawls. We ran four instances of OpenWPM crawlers that ran simultaneously visiting each website with a valid AAAA record. The distribution of Alexa top 10k websites that returned a valid AAAA DNS record is shown in \textbf{Figure 3}.    
\begin{figure}
\centering
        \includegraphics[totalheight=4cm]{images/Alexa_AAAA.png}
    \caption{Distribution of Alexa top 10k websites that returned a valid AAAA DNS record}
    \label{fig:verticalcell}
\end{figure}

\textbf{DNS open resolvers crawlers.} This experiment involved querying open DNS resolvers for an IPv6 domain. We collected a list of ~9k open DNS resolvers. These resolvers were queried simultaneously for the AAAA DNS record of \textit{www.google.com} using the 4 addresses allotted to this experiment. Each resolver was queried once every day (at most 3 times for a successful response) for the entirety of the experiment.

\textbf{NTP pool servers.} This experiment consisted of setting up 4 instances of NTP pool servers. \textit{should i put in stats about the pool servers  and the config?}

\textbf{NTP public servers.}

\textbf{Tor relays.} Talk about bandwidth? middle relay? People who used our relays? 

\textbf{DNS zone files.} To conduct this experiment, we set up 4 domains; 2 each with a \textit{.com} and \textit{.net} TLD. The AAAA records of all 4 domains were pointed to 4 distinct IPv6 addresses in our /56 IPv6 prefix. \textit{Should i explain here how dns zone files work?}


\subsection{Data collection}
Throughout the length of our experiment, we capture:
\begin{itemize}
	\item All network traffic destined for our /56 IPv6 prefix
	\item Logs of DNS PTR record queries made for IPs that reside inside our /56 IPv6 prefix
\end{itemize}   
We ran tcpdump to capture all traffic originating from and destined to our /56 IPv6 prefix. To collect DNS PTR record queries, we ran an authoritative DNS server which served all domains attached with our IP addresses with a TTL of 1. This made sure that most PTR record queries were not cached and indeed reached our DNS server.
\\  
Our dataset consists of ~5.2M unsolicited packets and ~600k unsolicited DNS PTR queries. Unsolicited traffic consists of all traffic that was not received as a result of any of our experiments and was generated by IP addresses that we never contacted throughout the entirety of our experiment. Unsolicited DNS PTR queries consist of all queries that were not sent in by hosts we contacted during our experimentation. We also exclude all DNS PTR queries that might have been generated due to the nature of our experiments \textit{i.e} NTP clients (or their firewalls) looking up the DNS PTR record of the NTP pool server they use \cite{poolntpo47:online}.  

